Emergent phenomena in QCD: The holographic perspective

A basic understanding of the relevant features of hadron properties from first principles QCD has remained elusive, and should be understood as emergent phenomena which depend critically on the number of dimensions of physical spacetime. These properties include the mechanism of color confinement, the origin of the hadron mass scale, chiral symmetry breaking and the pattern of hadronic bound states. Some of these complex issues have been recently addressed in an effective computational framework of hadron structure based on a semiclassical approximation to light-front QCD, and its holographic embedding in anti-de Sitter (AdS) space. This framework also embodies an underlying superconformal algebraic structure which gives rise to the emergence of a mass scale within the superconformal group: It determines the effective confinement potential of mesons, baryons and tetraquarks. The normalizable zero-mass ground state is identified with the pion which has no baryonic supersymmetric partner, a property which is shared for the lowest meson state in each particle family. This new approach to hadron physics leads to relativistic wave equations, similar in their simplicity to the Schroedinger equation in atomic physics, and provides important insights into the confinement mechanism of QCD.

==> biblio.tex <==
\begin{thebibliography}{62}

\small

\bibitem{Wilson:1974sk} 
K.~G.~Wilson, 
Confinement of quarks,
\href{https://doi.org/10.1103/PhysRevD.10.2445}{Phys. Rev. D \textbf {10}, 2445  (1974).}

\bibitem {Dirac:1949cp}
  P.~A.~M.~Dirac,  
  Forms of relativistic dynamics,
  \href{https://doi.org/10.1103/RevModPhys.21.392}{Rev. Mod. Phys. \textbf{21}, 392 (1949).}

\bibitem{Kreshchuk:2020dla}
M.~Kreshchuk, W.~M.~Kirby, G.~Goldstein, H.~Beauchemin and P.~J.~Love,
Quantum simulation of quantum field theory in the light-front formulation,
\href{https://doi.org/10.1103/PhysRevA.105.032418}{Phys. Rev. A \textbf{105}, 032418 (2022)}
[\href{https://arxiv.org/abs/2002.04016}{\tt arXiv:2002.04016 [quant-ph]}].


\bibitem{Gross:2022hyw}
F.~Gross, E.~Klempt, S.~J.~Brodsky, A.~J.~Buras, V.~D.~Burkert, G.~Heinrich, K.~Jakobs, C.~A.~Meyer, K.~Orginos and M.~Strickland, \textit{et al.},
50 Years of Quantum Chromodynamics,
[\href{https://arxiv.org/abs/2212.11107}{\tt arXiv:2212.11107 [hep-ph]}].


\bibitem{Maldacena:1997re}
J.~M.~Maldacena,  
The large-$N$ limit of superconformal field theories and supergravity,
\href{https://doi.org/10.1023/A:1026654312961} {Adv. Theor. Math. Phys. \textbf{2}, 231 (1998)}
[\href{https://arxiv.org/abs/hep-th/9711200} {\tt arXiv:hep-th/9711200}].


 \bibitem{Gubser:1998bc}
  S.~S.~Gubser, I.~R.~Klebanov and A.~M.~Polyakov,
  Gauge theory correlators from non-critical string theory,
  \href{http://www.sciencedirect.com/science/article/pii/S0370269398003773}{Phys.\ Lett.\ B {\bf 428}, 105 (1998)}
  [\href{http://arXiv.org/abs/hep-th/9802109}{\tt arXiv:hep-th/9802109}].


\bibitem{Witten:1998qj}
  E.~Witten,
  Anti-de Sitter space and holography,
  Adv.\ Theor.\ Math.\ Phys.\  {\bf 2}, 253 (1998)
  [\href{http://arXiv.org/abs/hep-th/9802150}{\tt arXiv:hep-th/9802150}].


\bibitem{Aharony:1999ti}
   O.~Aharony,    S.~S.~Gubser, J.~M.~Maldacena, H.~Ooguri, and  Y.~ Oz, 
   Large $N$ field theories, string theory and gravity, 
   \href{https://doi.org/10.1016/S0370-1573(99)00083-6}{Phys. Rept. \textbf{323}, 183 (2000)}
[\href{https://arxiv.org/abs/hep-th/9905111} {\tt arXiv:hep-th/9905111}].

\bibitem{deTeramond:2008ht}
  G.~F.~de~T\'eramond and   S.~J. Brodsky,  
  Light-front holography: A first approximation to QCD, 
  \href{https://doi.org/10.1103/PhysRevLett.102.081601}{Phys. Rev. Lett. \textbf{102}, 081601 (2009)}
  [\href{https://arxiv.org/abs/0809.4899}{\tt arXiv:0809.4899 [hep-ph]}].
  
\bibitem{deTeramond:2013it}
  G.~F. de~T\'eramond,  H.~G.~Dosch, and   S.~J.~Brodsky,  
  Kinematical and dynamical aspects of higher-spin bound-state equations in holographic QCD,
  \href{https://doi.org/10.1103/PhysRevD.87.075005}{Phys. Rev. D \textbf {87}, 075005 (2013)}
  [\href{https://arxiv.org/abs/1301.1651} {\tt arXiv:1301.1651 [hep-ph]}].
  
\bibitem{Brodsky:2014yha}
  S.~J.~Brodsky,  G.~F.~de~T\'eramond,   H.~G.~Dosch, and  J.~Erlich,  
  Light-front holographic QCD and emerging confinement, 
  \href{https://doi.org/10.1016/j.physrep.2015.05.001}{Phys. Rept. \textbf{584}, 1 (2015)}
  [\href{https://arxiv.org/abs/1407.8131}{\tt arXiv:1407.8131 [hep-ph]}].

\bibitem{Polchinski:2002jw}
  J.~Polchinski and  M.~J.~Strassler,  
  Deep inelastic scattering and gauge/string duality, 
  \href{https://doi.org/10.1088/1126-6708/2003/05/012}{JHEP  \textbf{05}, 012 (2003)}
  [\href{https://arxiv.org/abs/hep-th/0209211}{\tt arXiv:hep-th/0209211}].
  
\bibitem {Brodsky:2006uqa}
  S.~J.~Brodsky and   G.~F.~de~T\'eramond,  
  Hadronic spectra and light-front wave functions in holographic QCD,  
  \href{https://doi.org/10.1103/PhysRevLett.96.201601}{Phys. Rev. Lett. \textbf  {96},  201601 (2006)}
  [\href{https://arxiv.org/abs/hep-ph/0602252} {\tt arXiv:hep-ph/0602252}].
 
\bibitem{deAlfaro:1976vlx}
   V.~de~Alfaro,  S.~ Fubini,  and   G.~ Furlan,
   Conformal invariance in quantum mechanics,  
   \href{https://doi.org/10.1007/BF02785666}{Nuovo Cim. A \textbf{34}, 569 (1976).}
  
\bibitem{Fubini:1984hf}
   S.~Fubini and  E.~Rabinovici,  
   Superconformal quantum mechanics,  
   \href{https://doi.org/10.1016/0550-3213(84)90422-X}{Nucl. Phys. B \textbf{245}, 17 (1984).}

\bibitem{Akulov:1983hjq}
  V.~P.~Akulov  and   A.~I.~Pashnev,  
  Quantum superconformal model in $(1,2)$ space,  
  \href{https://doi.org/10.1007/BF01086252}{Theor. Math. Phys. \textbf{56}, 862 (1983).}  

\bibitem{Brodsky:2013ar}
  S.~J.~Brodsky,    G.~F.~de~T\'eramond,  and   H.~G.~Dosch,  
  Threefold complementary approach to holographic QCD,  
  \href{https://doi.org/10.1016/j.physletb.2013.12.044}{Phys. Lett. B \textbf{729}, 3 (2014)}
  [\href{https://arxiv.org/abs/1302.4105} {\tt arXiv:1302.4105 [hep-th]}].
  
\bibitem{deTeramond:2014asa}
  G.~F.~de~T\'eramond,  H.~G.~Dosch, and  S.~J.~Brodsky,  
  Baryon spectrum from superconformal quantum mechanics and its light-front holographic embedding,  
  \href{https://doi.org/10.1103/PhysRevD.91.045040} {Phys. Rev. D \textbf {91}, 045040 (2015)} 
  [\href{https://arxiv.org/abs/1411.5243} {\tt arXiv:1411.5243 [hep-ph]}].
  
\bibitem{Dosch:2015nwa}
  H.~G.~Dosch,   G.~F. de~T\'eramond, and  S.~J.~Brodsky, 
  Superconformal baryon-meson symmetry and light-front holographic QCD,
   \href{https://doi.org/10.1103/PhysRevD.91.085016}{Phys. Rev. D \textbf{91}, 085016 (2015)}
   [\href{https://arxiv.org/abs/1501.00959}{\tt arXiv:1501.00959 [hep-th]}].
   
 \bibitem{deTeramond:2018ecg} 
  G.~F.~de T\'eramond, T.~Liu, R.~S.~Sufian,  H.~G.~Dosch, S.~J.~Brodsky and A.~Deur [HLFHS],
  Universality of generalized parton distributions in light-front holographic QCD,
  \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.120.182001}{Phys.\ Rev.\ Lett.\  {\bf 120},  182001 (2018)}
  [\href{https://arxiv.org/abs/1801.09154}{\tt arXiv:1801.09154 [hep-ph]}].
  
 \bibitem{Liu:2019vsn} 
  T.~Liu, R.~S.~Sufian, G.~F.~de T\'eramond, H.~G.~Dosch, S.~J.~Brodsky and A.~Deur [HLFHS],
  Unified description of polarized and unpolarized quark distributions in the proton,
  \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.124.082003}{Phys.\ Rev.\ Lett.\  {\bf 124},  082003 (2020)}
  [\href{https://arxiv.org/abs/1909.13818}{\tt arXiv:1909.13818 [hep-ph]}].

\bibitem{deTeramond:2021lxc}
G.~F.~de T\'eramond, H.~G.~Dosch, T.~Liu, R.~S.~Sufian,   S.~J.~Brodsky and A.~Deur [HLFHS],
Gluon matter distribution in the proton and pion from extended holographic light-front QCD,
\href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.104.114005}{Phys. Rev. D \textbf{104}, 114005 (2021)}
[\href{https://arxiv.org/abs/2107.01231}{\tt arXiv:2107.01231 [hep-ph]}].
   
\bibitem{deTeramond:2022int}
  G.~F. de~T\'eramond,
Emergent phenomena in nonperturbative QCD: The holographic light-front perspective,  
In \href{https://www.int.washington.edu/sites/default/files/schedule_session_files/deTeramond.pdf}{\it Origin of the Visible Universe: Unraveling the Proton Mass}, INT Seattle, 13-17 June 2022.

\bibitem{Pauli:1985pv}
H.~C.~Pauli and S.~J.~Brodsky,
Solving field theory in one space and one time dimension,
\href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.32.1993}{Phys. Rev. D \textbf{32}, 1993 (1985)}.

\bibitem{Hornbostel:1988ne}
K.~Hornbostel,
The application of light cone quantization to quantum chromodynamics in one-plus-one dimensions,
Ph.~D. thesis Stanford University, 
\href{https://inspirehep.net/files/5382bfadf6016c08e11430938dd83262}{SLAC-PUB-0333 (1988)}.  
       
\bibitem{Gross:1973id} 
  D.~J.~Gross and F.~Wilczek,
  Ultraviolet behavior of non abelian gauge theories,
 \href{http://prl.aps.org/abstract/PRL/v30/i26/p1343_1}{Phys.\ Rev.\ Lett.\  {\bf 30}, 1343 (1973)}.
 
\bibitem{Politzer:1973fx} 
  H.~D.~Politzer,
  Reliable perturbative results for strong interactions?,
\href{http://prl.aps.org/abstract/PRL/v30/i26/p1346_1}{Phys.\ Rev.\ Lett.\  {\bf 30}, 1346 (1973)}.    
   
\bibitem{tHooft:1974pnl}
G.~'t Hooft,
A two-dimensional model for mesons,
\href{https://www.sciencedirect.com/science/article/abs/pii/0550321374900881?via%3Dihub}{Nucl. Phys. B \textbf{75}, 461 (1974)}.   

\bibitem{Hornbostel:1988fb}
K.~Hornbostel, S.~J.~Brodsky and H.~C.~Pauli,
Light-cone-quantized QCD in 1+1 dimensions,
\href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.41.3814}{Phys. Rev. D \textbf{41}, 3814 (1990)}.

\bibitem{Eller:1986nt}
T.~Eller, Ph.~D. thesis Heidelberg University, unpublished;
T.~Eller, H.~C.~Pauli and S.~J.~Brodsky,
Discretized light cone quantization: The massless and the massive Schwinger model,
\href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.35.1493}{Phys. Rev. D \textbf{35}, 1493 (1987)}.

\bibitem{Demeterfi:1993rs}
K.~Demeterfi, I.~R.~Klebanov and G.~Bhanot,
Glueball spectrum in a (1+1)-dimensional model for QCD,
\href{https://www.sciencedirect.com/science/article/abs/pii/0550321394902364?via%3Dihub}{Nucl. Phys. B \textbf{418}, 15 (1994)}
[\href{https://arxiv.org/abs/hep-th/9311015}{\tt arXiv:hep-th/9311015 [hep-th]}]. 


\bibitem{Polchinski:2001tt}
  J.~Polchinski and M.~J.~Strassler,
 Hard scattering and gauge/string duality,
  \href{http://prl.aps.org/abstract/PRL/v88/i3/e031601}{Phys.\ Rev.\ Lett.\  {\bf 88}, 031601 (2002)}
  [\href{http://arXiv.org/abs/hep-th/0109174}{\tt arXiv:hep-th/0109174}].
  

  \bibitem{Karch:2006pv}
  A.~Karch, E.~Katz, D.~T.~Son and M.~A.~Stephanov,
  Linear confinement and AdS/QCD,
 \href{http://prd.aps.org/abstract/PRD/v74/i1/e015005}{ Phys.\ Rev.\  D {\bf 74}, 015005 (2006)}
  [\href{http://arXiv.org/abs/hep-ph/0602229}{\tt arXiv:hep-ph/0602229}].
  
 
  \bibitem{Kirsch:2006he} 
  I.~Kirsch,
  Spectroscopy of fermionic operators in AdS/CFT,
  \href{http://iopscience.iop.org/1126-6708/2006/09/052/}{JHEP\ {\bf 0609}, 052  (2006)}
  [\href{http://arXiv.org/abs/hep-th/0607205}{\tt arXiv:hep-th/0607205}].

 
   \bibitem{Abidin:2009hr}   
  Z.~Abidin and C.~E.~Carlson,
  Nucleon electromagnetic and gravitational form factors from holography,
 \href{http://prd.aps.org/abstract/PRD/v79/i11/e115003}{Phys.\ Rev.\  D {\bf 79}, 115003 (2009)}
  [\href{http://arXiv.org/abs/0903.4818}{\tt arXiv:0903.4818 [hep-ph]}]. 


 \bibitem{Gutsche:2011vb}
  T.~Gutsche, V.~E.~Lyubovitskij, I.~Schmidt and A.~Vega,
  Dilaton in a soft-wall holographic approach to mesons and baryons,
  \href{http://prd.aps.org/abstract/PRD/v85/i7/e076003}{ Phys.\ Rev.\ D {\bf 85}, 076003 (2012)}
  [\href{http://arXiv.org/abs/1108.0346}{\tt arXiv:1108.0346 [hep-ph]}].
  
  
\bibitem {Witten:1981nf}
  E.~Witten,  Dynamical breaking of supersymmetry,  
  \href{https://doi.org/10.1016/0550-3213(81)90006-7}{Nucl. Phys. B \textbf{188}, 513 (1981).}
  
\bibitem{Miyazawa:1966mfa}
   H.~Miyazawa,  
   Baryon number changing currents,  
   \href{https://doi.org/10.1143/PTP.36.1266}{Prog. Theor. Phys. \textbf{36}, 1266 (1966).}

\bibitem{Catto:1984wi}
   S.~Catto and F.~ Gursey,
   Algebraic treatment of effective supersymmetry, 
    \href{https://doi.org/10.1007/BF02902548}{Nuovo Cim. A  \textbf{86}, 201 (1985).}
  
\bibitem{Lichtenberg:1999sc}
  D.~B.~Lichtenberg,  
  Whither hadron supersymmetry?, in {\it International Conference on Orbis Scientiae 1999: Quantum Gravity,
  Generalized Theory of Gravitation and Superstring Theory Based Unification},
  28th Conference on High-Energy Physics and Cosmology  (1999) pp. 203--208, 
  \href{https://arxiv.org/abs/hep-ph/9912280}{\tt arXiv:hep-ph/9912280.}

\bibitem{ParticleDataGroup:2022pth}
R.~L.~Workman \textit{et al.} [Particle Data Group],
Review of particle physics,
\href{https://doi.org/10.1093/ptep/ptac097}{PTEP  \textbf{2022}, 083C01 (2022).}


\bibitem{Dosch:2016zdv}
H.~G.~Dosch, G.~F.~de T\'eramond and S.~J.~Brodsky,
Supersymmetry across the light and heavy-light Hadronic Spectrum II,
\href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.95.034016}{Phys. Rev. D \textbf{95}, 034016 (2017)}
[\href{https://arxiv.org/abs/1612.02370}{\tt arXiv:1612.02370 [hep-ph]}].


\bibitem{Brodsky:2016yod}
  S.~J.~Brodsky,  G.~F.~de~T\'eramond,   H.~G.~Dosch, and   C.~Lorc\'e,  
  Universal effective hadron dynamics from superconformal algebra,  
  \href{https://doi.org/10.1016/j.physletb.2016.05.068}{Phys. Lett. B \textbf{759} 171 (2016)}
 [\href{https://arxiv.org/abs/1604.06746}{\tt arXiv:1604.06746 [hep-ph]}].
 
\bibitem{Erlich:2005qh}
  J.~Erlich,  E.~ Katz, D.~T.~Son, and  M.~A.~Stephanov,
   QCD and a holographic model of hadrons,  
   \href{https://doi.org/10.1103/PhysRevLett.95.261602}{Phys. Rev. Lett.  \textbf  {95}, 261602 (2005)}
 [\href{https://arxiv.org/abs/hep-ph/0501128}{\tt arXiv:hep-ph/0501128}].
  
\bibitem{DaRold:2005mxj}
   L.~Da~Rold and  A.~Pomarol,  
   Chiral symmetry breaking from five-dimensional spaces,  
   \href{https://doi.org/10.1016/j.nuclphysb.2005.05.009}{Nucl. Phys. B \textbf{72}, 79 (2005)}
  [\href{https://arxiv.org/abs/hep-ph/0501218}{\tt arXiv:hep-ph/0501218}].
  
  
\bibitem{deTeramond:2021yyi}
G.~F.~de T\'eramond and S.~J.~Brodsky,
Longitudinal dynamics and chiral symmetry breaking in holographic light-front QCD,
\href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.104.116009}{Phys. Rev. D \textbf{104}, 116009 (2021)}
[\href{https://arxiv.org/abs/2103.10950}{\tt arXiv:2103.10950 [hep-ph]}].


\bibitem{Li:2022izo}
Y.~Li and J.~P.~Vary,
Longitudinal dynamics for mesons on the light cone,
\href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.105.114006}{Phys. Rev. D \textbf{105}, 114006 (2022)}
[\href{https://arxiv.org/abs/2202.05581}{\tt arXiv:2202.05581 [hep-ph]}].


\bibitem{Dosch:2020hqm}
   H.~G.~Dosch, S.~J.~Brodsky, G.~F.~de~T\'eramond, M.~Nielsen, and L.~ Zou,  
   Exotic states in a holographic theory,  
   \href{https://doi.org/10.1016/j.nuclphysbps.2021.05.035}{Nucl. Part. Phys. Proc. \textbf{312-317}, 135 (2021)} 
   [\href{https://arxiv.org/abs/2012.02496}{\tt arXiv:2012.02496 [hep-ph]}].


\bibitem{Dosch:2015bca}
  H.~G. Dosch,  G.~F.~de~T\'eramond, and S.~J.~Brodsky, 
  Supersymmetry across the light and heavy-light hadronic spectrum,  
  \href{https://doi.org/10.1103/PhysRevD.92.074010}{Phys. Rev. D \textbf {92}, 074010 (2015)}
  [\href{https://arxiv.org/abs/1504.05112}{\tt arXiv:1504.05112 [hep-ph]}].
  
  
\bibitem{Shuryak:1981fza}
E.~V.~Shuryak,
Hadrons containing a heavy quark and QCD sum rules,
\href{https://www.sciencedirect.com/science/article/abs/pii/0550321382905466?via%3Dihub}{Nucl. Phys. B \textbf{198}, 83 (1982)}.


\bibitem{Isgur:1991wq}
N.~Isgur and M.~B.~Wise,
Spectroscopy with heavy-quark symmetry,
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.66.1130}{Phys. Rev. Lett. \textbf{66}, 1130 (1991)}.


\bibitem{Gutsche:2012ez}
T.~Gutsche, V.~E.~Lyubovitskij, I.~Schmidt and A.~Vega,
Chiral symmetry breaking and meson wave functions in soft-wall AdS/QCD,
\href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.87.056001}{Phys. Rev. D \textbf{87}, 056001 (2013)}
[\href{https://arxiv.org/abs/1212.5196}{\tt arXiv:1212.5196 [hep-ph]}].

  
 \bibitem{Nielsen:2018ytt}
  M.~Nielsen,  S.~J.~Brodsky,  G.~F.~de~T\'eramond,  H.~G.~Dosch,  F.~S.~Navarra, and L.~ Zou, 
   Supersymmetry in the double-heavy hadronic spectrum,  
   \href{https://doi.org/10.1103/PhysRevD.98.034002}{Phys. Rev. D \textbf{98}, 034002 (2018)}
  [\href{https://arxiv.org/abs/1805.11567}{\tt arXiv:1805.11567 [hep-ph]}]. 
  
  
  \bibitem{Nielsen:2018uyn}
  M.~Nielsen and  S.~J.~Brodsky,  
  Hadronic superpartners from a superconformal and supersymmetric algebra, 
  \href{https://doi.org/10.1103/PhysRevD.97.114001}{Phys. Rev. D \textbf{97}, 114001 (2018)}
  [\href{https://arxiv.org/abs/1802.09652}{\tt arXiv:1802.09652 [hep-ph]}].

  
\bibitem{Karliner:2017qjm}
  M.~Karliner and  J.~L. Rosner,  Discovery of doubly-charmed $\Xi_{cc}$ baryon implies a stable $b b \bar{u} \bar{d}$ tetraquark,   
  \href{https://doi.org/10.1103/PhysRevLett.119.202001}{Phys. Rev. Lett \textbf{119}, 202001 (2017)}
  [\href{https://arxiv.org/abs/1707.07666} {\tt arXiv:1707.07666 [hep-ph]}].
 
    
\bibitem{LHCb:2021vvq}
R.~Aaij \textit{et al.} [LHCb],
Observation of an exotic narrow doubly charmed tetraquark,
\href{https://doi.org/10.1038/s41567-022-01614-y}{Nature Phys. \textbf{18}, 751-754 (2022)}
[\href{https://arxiv.org/abs/2109.01038}{\tt arXiv:2109.01038 [hep-ex]}].   


\bibitem{Sufian:2018cpj}
R.~S.~Sufian, T.~Liu, G.~F.~de T\'eramond, H.~G.~Dosch, S.~J.~Brodsky, A.~Deur, M.~T.~Islam and B.~Q.~Ma,
Nonperturbative strange-quark sea from lattice QCD, light-front holography, and meson-baryon fluctuation models,
\href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.98.114004}{Phys. Rev. D \textbf{98}, 114004 (2018)}
\href{https://arxiv.org/abs/1809.04975}{[\tt arXiv:1809.04975 [hep-ph]}].


\bibitem{Sufian:2020coz}
R.~S.~Sufian, T.~Liu, A.~Alexandru, S.~J.~Brodsky, G.~F.~de T\'eramond, H.~G.~Dosch, T.~Draper, K.-F.~Liu and Y.-B.~Yang,
Constraints on charm-anticharm asymmetry in the nucleon from lattice QCD,
\href{https://doi.org/10.1016/j.physletb.2020.135633}{Phys. Lett. B \textbf{808}, 135633 (2020)}
[\href{https://arxiv.org/abs/2003.01078}{\tt arXiv:2003.01078 [hep-lat]}].


\bibitem{Deur:2022msf}
A.~Deur, V.~Burkert, J.~P.~Chen and W.~Korsch,
Experimental determination of the QCD effective charge $\alpha_{g_1}(Q)$,
\href{https://www.mdpi.com/2571-712X/5/2/15}{Particles \textbf{5}, 171 (2022)}
[\href{https://arxiv.org/abs/2205.01169}{\tt arXiv:2205.01169 [hep-ph]}].


\bibitem{Brodsky:2022bum}
S.~J.~Brodsky and G.~F.~de T\'eramond,
Onset of color transparency in holographic light-front QCD,
\href{https://www.mdpi.com/2624-8174/4/2/42}{MDPI Physics \textbf{4},  633 (2022)}
[\href{https://arxiv.org/abs/2202.13283}{\tt arXiv:2202.13283 [hep-ph]}].


\bibitem{Forshaw:2012im}
J.~R.~Forshaw and R.~Sandapen,
An AdS/QCD holographic wave unction for the $\rho$ meson and diffractive $\rho$ meson electroproduction,
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.109.081601}{Phys. Rev. Lett. \textbf{109}, 081601 (2012)}
[\href{https://arxiv.org/abs/1203.6088}{\tt arXiv:1203.6088 [hep-ph]}].


\bibitem{Kim:2022lng}
D.~N.~Kim and G.~A.~Miller,
Light-front holography model of the EMC effect,
\href{https://journals.aps.org/prc/abstract/10.1103/PhysRevC.106.055202}{Phys. Rev. C \textbf{106},  055202 (2022)}
[\href{https://arxiv.org/abs/2209.13753}{\tt arXiv:2209.13753 [nucl-th]}].


\end{thebibliography}
